DrivingDojo Dataset: Advancing Interactive and Knowledge-Enriched Driving World Model

Driving world models have gained increasing attention due to their ability to model complex physical dynamics. However, their superb modeling capability is yet to be fully unleashed due to the limited video diversity in current driving datasets. We introduce DrivingDojo, the first dataset tailor-made for training interactive world models with complex driving dynamics. Our dataset features video clips with a complete set of driving maneuvers, diverse multi-agent interplay, and rich open-world driving knowledge, laying a stepping stone for future world model development. We further define an action instruction following (AIF) benchmark for world models and demonstrate the superiority of the proposed dataset for generating action-controlled future predictions.

==> figs/action_cases.tex <==
\begin{figure}[htbp]
  \centering
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{imgs/NaVI_Demo_action.pdf}
    \caption{Examples of rich ego actions}
     \label{fig:actions}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{imgs/NaVI_Demo_interact.pdf}
    \caption{Examples of multi-agent interplay}
    \label{fig:interaction}
    \end{subfigure}
\caption{
(a) Row 1: Illustration of a lane change. Row 2: Showing a hard brake and stop when facing traffic control.Row 3: Turning at a crossing. (b) Row 1: Blocked by the pedestrian and motorcycle. Row 2: Blocked by the vehicle and failed cutting in. Row 3: cutting off and successful cutting in.
}
\end{figure}

==> figs/demo_generalization.tex <==
\begin{figure}[htbp]
  \centering
    \includegraphics[width=1.0\textwidth]{imgs/generalization.pdf} 
  \caption{\textbf{Model generalization capability.} Row 1 and Row 2 demonstrate out-of-domain actions on our dataset. Row 3 and Row 4 show generalization to other datasets, such as lane changes on OpenDV-2K and backing up on nuScenes.}
  \label{fig:action_generalization}
  \vspace{-10pt}
\end{figure}


==> figs/demo_interaction.tex <==
\begin{figure}[htbp]
  \centering
   \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{imgs/interaction.pdf}
    \caption{Multi-agent interplay simulation}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{imgs/rare.pdf}
    \caption{Open-world dynamics}
    \end{subfigure}
  \caption{\textbf{Interaction simulation.}}
  \label{fig:interaction_demo}
\end{figure}

==> figs/diverse_case.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\textwidth]{imgs/NaVI_diverse_case.pdf} 
  \caption{\textbf{Examples of diverse and rare cases in our dataset.}}
  \label{fig:diverse}
\end{figure}


==> figs/interaction.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\textwidth]{imgs/NaVI_Demo_interact.pdf} 
  \caption{\textbf{Examples of multi-agent interplay.} Row 1: Blocked by the pedestrian and motorcycle. Row 2: Blocked by the vehicle and failed cutting in. Row 3: cutting off and successful cutting in.}
  \label{fig:interaction}
  \vspace{-10pt}
\end{figure}

==> figs/latent_knowledge.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\textwidth]{imgs/NaVI_Demo_latent.pdf} 
  \caption{Examples of latent knowledge include:
(a) Illustration of a vehicle encountering a red light and coming to a stop.
(b) Illustration of a vehicle starting when the traffic light turns green.
(c) and (d) Illustration of a vehicle encountering a boom barrier.
}
  \label{fig:knowledge}
\end{figure}



==> figs/ood.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{imgs/NaVI_Demo_ood.pdf}
    \caption{Examples of rich open-world knowledge.}
  \label{fig:ood}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{imgs/NaVI_diverse_case}
    \caption{Examples of diverse and rare cases in our dataset.}
    \label{fig:diverse}
    \end{subfigure}
  \caption{(a)
Row 1: Displays of encountering rolling objects.
Row 2: Displays of encountering falling objects.
Row 3: Displays of encountering moving or floating unknown objects.
Row 4: Displays of facing traffic lights and boom barriers.}
  \vspace{-10pt}
\end{figure}


==> sec/5_discuss.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Limitations and Future Work}
\label{sec:limitation}
However, our model has a few limitations that call for future work.

\noindent{\textbf{Hallucination.}}
As shown in Figure~\ref{fig:hallucination}, when an action is unrealistic given the scene, the experiment finds that the model exhibits some hallucinations, such as creating new roads.
\input{figs/hallucination}

\noindent{\textbf{Long-horizon Visual Prediction.}
Our baseline model is only capable of generating short videos, which can be used to simulate short-term interaction events. 
Longer predictions~\cite{henschel2024streamingt2v} and faster generation~\cite{meng2023distillation,luo2023latent} speeds are left for future research.

\subsection{Societal Impacts}
\label{sec:social}
The development of world model requires large and diverse driving videos, introducing privacy issues. By providing a comprehensive dataset covering diverse driving scenarios and behaviors, researchers can develop and refine algorithms that increase the safety, reliability, and efficiency of autonomous vehicles. 
